Minimizing the Sum of Age of Information and Transmission Cost under Stochastic Arrival Model

We consider a node-monitor pair, where updates are generated stochastically (according to a known distribution) at the node that it wishes to send to the monitor. The node is assumed to incur a fixed cost for each transmission, and the objective of the node is to find the update instants so as to minimize a linear combination of AoI of information and average transmission cost. First, we consider the Poisson arrivals case, where updates have an exponential inter-arrival time for which we derive an explicit optimal online policy. Next, for arbitrary distributions of inter-arrival time of updates, we propose a simple randomized algorithm that transmits any newly arrived update with a fixed probability (that depends on the distribution) or never transmits that update. The competitive ratio of the proposed algorithm is shown to be a function of the variance and the mean of the inter-arrival time distribution. For some of the commonly considered distributions such as exponential, uniform, and Rayleigh, the competitive ratio bound is shown to be 2.

==> Abstract.tex <==
We consider a node-monitor pair, where updates are generated stochastically (according to a known distribution) at the node that it wishes tosend to the server. The node is assumed to incur a fixed cost for each transmission, and the objective of the node is to find the update instants so as to minimize a linear combination of age of information and average transmission cost. 
First, we consider the Poisson arrivals case, where updates have an exponential inter-arrival time for which we derive an explicit optimal online policy. 
Next, for arbitrary distributions of inter-arrival time of updates, we propose a simple randomized algorithm that transmits any newly arrived update with a fixed probability (that depends on the distribution) or never transmits that update. The competitive ratio of the proposed algorithm is shown to be a function of the variance and the mean of the inter-arrival time distribution. For some of the commonly considered distributions such as exponential, uniform, and Rayleigh, the competitive ratio bound is 2.

%We consider a node-server pair, where the server seeks regular updates from the node to minimize its age of information. However, at the node, the updates are generated stochastically (according to a known distribution), and the node incurs a fixed cost for each transmitted packet. 
%Hence, there is a need for a causal transmission policy that could simultaneously minimize both average age and average transmission cost, which is in general, conflicting in nature. In this paper, we find such a transmission policy by formulating the given tradeoffs as an optimization problem, where the objective is to minimize the sum of average age and average transmission cost over the set of causal transmission policies. To start with, we assume that the packets are generated according to a Poisson distribution, and find a threshold policy that is optimal among all the threshold policies that minimize the sum of average age and average transmission cost. We then generalize the result to general distributions over the packet generation process by proposing a stationary randomized transmission policy and computing a competitive ratio for the policy that is bounded for most practical distributions over the packet generation process.

%We consider a node-server pair, where the server seeks regular updates from the node to minimize its age of information. However, the updates are generated at the node stochastically (according to a known distribution), and the node incurs a fixed cost for each transmitted packet. 
%Hence, there is need for a causal transmission policy that could simultaneously minimize both age and transmission cost, that is in general, conflicting in nature. In this paper, we find such a transmission policy by formulating the given tradeoffs as an optimization problem, where the objective is to minimize the sum of average age and average transmission cost over all causal transmission policies. To start with, we that the packets are generated according to a poisson distribution, and find a threshold policy that that is optimal among all the threshold policies that minimizes the sum of average age and average transmission cost. We then generalize the result to general distributions over packet generation process by proposing a stationary randomized transmission policy, and computing a competitive ratio for the policy that is bounded for most practical distributions over packet generation process.

% where packets are generated according to a known distribution. The packets are to be transmitted to a serverThe node wants to minimize its age by transmitting the packets to the server
